LLM4GRN: Discovering Causal Gene Regulatory Networks with LLMs -- Evaluation through Synthetic Data Generation

Gene regulatory networks (GRNs) represent the causal relationships between transcription factors (TFs) and target genes in single-cell RNA sequencing (scRNA-seq) data. Understanding these networks is crucial for uncovering disease mechanisms and identifying therapeutic targets. In this work, we investigate the potential of large language models (LLMs) for GRN discovery, leveraging their learned biological knowledge alone or in combination with traditional statistical methods. We develop a task-based evaluation strategy to address the challenge of unavailable ground truth causal graphs. Specifically, we use the GRNs suggested by LLMs to guide causal synthetic data generation and compare the resulting data against the original dataset. Our statistical and biological assessments show that LLMs can support statistical modeling and data synthesis for biological research.

==> preliminaries.tex <==
\section{Preliminaries}\label{app:preliminaries}

% \subsection{Causal Graph}\label{DAG}

% A directed acyclic graph (DAG) $\mathcal{G} = (\mathbf{V},\mathcal{E})$ is composed of a set of variables/vertices $\mathbf{V}$ and a set of (directed) edges $\mathcal{E}$ between them such that no cycle is formed.
% Let $P$ be the probability distribution over the same set of variables $\mathbf{V}$.
% $\mathcal{G}$ and $P$ satisfy the Markov condition if every variable is conditionally independent of its non-descendants given its parents.
% Assuming the Markov condition, the joint distribution of variables $V_1,V_2,\ldots \in \mathbf{V}$ can be factorized as:
% \begin{equation}
%     P[V_1,V_2,\ldots, V_d] = \prod_{i}P[V_i | Pa(V_i)] \label{eq:markov}\ .
% \end{equation}
% where $Pa(V_i)$ denotes the set of parents of $V_i$.

\subsection{Gene Regulatory Network}\label{GRN}

A gene regulatory network (GRN) is a collection of molecular regulators that interact with each other and with other substances in the cell to control the gene expression levels of mRNA and proteins. GRNs describe the relationships between genes, transcription factors, RNA molecules, and other regulatory elements within a biological system, illustrating how genes are turned on or off and how their expression is modulated over time and in different conditions. GRN can be expressed as a directed acyclic graph (DAG)~\ref{DAG}. In this work we are considering a two layer DAG consisting of transcription factors (TFs) and target genes. TFs are proteins that bind to specific DNA sequences to regulate the transcription and influence the expression levels of target genes. GRNs are crucial for understanding how cells respond to changes in their environment, how different cell types develop, and how malfunctions in these networks can lead to diseases like cancer or Alzheimer's disease.

\subsection{GroundGan}\label{GroundGan}

GRouNdGAN~\cite{zinati2024groundgan} is a deep learning model that generates simulated single-cell RNA-seq data by leveraging causal generative adversarial networks (CausalGAN) and imposed user-defined causal gene regulatory networks (GRNs). The model comprises a causal controller, target generators, a critic, a labeler, and an anti-labeler, each implemented as separate neural networks. Training involves two steps: pre-training the causal controller using a Wasserstein GAN (WGAN) to generate TF expression values resembling reference data, followed by training the target generators to produce target gene expressions based on these TF values and random noise. The generated expressions undergo library-size normalization (LSN). The critic quantifies the Wasserstein distance between reference and simulated data, while the target generators are adversarially trained to generate realistic data points. The labeler and anti-labeler ensure that target gene expressions encode regulatory information from TFs.

\subsection{GRNBoost2}\label{GRNBoost2}

GRNBoost2~\cite{moerman2019grnboost2} is a scalable algorithm for inferring gene regulatory networks (GRNs) from single-cell RNA sequencing (scRNA-seq) data. It is part of the arboreto framework and is widely used due to its efficiency and scalability, especially for large datasets. GRNBoost2 employs gradient boosting, a machine learning method, to model the relationships between transcription factors (TFs) and target genes.
